Unconventional Superconductivity in Correlated, Multiband, and Topological Systems

In this thesis, we theoretically examine the pairing mechanisms and the identification of the pairing symmetry of unconventional superconductors whose normal states are correlated, multiband, or topological. In the first part, we investigate whether fluctuating intra-unit-cell loop currents can drive unconventional superconductivity. For general systems, we find that even-parity loop currents are not an effective pairing glue, whereas odd-parity loop currents, such as those proposed to explain the cuprates, are strong pair-breakers, suppressing rather than enhancing Cooper pairing. By employing the same methodology, we also analyze quantum-critical pairing due to other intra-unit-cell orders. For cuprates, we review the evidence for intra-unit-cell loop currents in the pseudogap, we classify the possible loop-current and particle-hole orders in the Emery model, and we analyze the pairing due to the various possible loop-current orders. In the second part, we present a novel electronic pairing mechanism that is based on electric monopole-dipole interactions. We show that these interactions become enhanced in quasi-2D systems with strong parity-mixing and spin-orbit coupling, such as doped Bi$_2$Se$_3$ or SnTe, and that they induce unconventional odd-parity superconductivity. In addition, we establish that the proposed pairing glue is measurable in the out-of-plane optical conductivity. In the last part, we reexamine the pairing symmetry of Sr$_2$RuO$_4$ in light of recent experiments. By theoretically analyzing recent $T_c$ and elastocaloric measurements under uniaxial stress, we demonstrate that the pairing state includes $s$, $d_{x^2-y^2}$, or body-centered $d_{xz} + i d_{yz}$ admixtures and that a bulk two-component superconductivity requires a great deal of fine-tuning to be consistent with ultrasound experiments.

==> Macros/layout.tex <==

\renewcommand{\sfdefault}{phv} % sets Helvetica as the default sans font

\makeatletter
\usepackage{etoolbox}
\pretocmd{\tableofcontents}{%
  \if@openright\cleardoublepage\else\clearpage\fi
  \pdfbookmark[0]{\contentsname}{toc}%
}{}{}%
\makeatother
% https://tex.stackexchange.com/questions/1820/contents-in-pdf-bookmarks

\setcounter{secnumdepth}{3} % makes the subsubsections numbered as well
\setcounter{tocdepth}{3} % adds them to the table of contents

% defines fancy chapter titles, in black
\colorlet{chapcolor}{black}
\addtokomafont{chapter}{\color{chapcolor}}
\makeatletter
\renewcommand*{\chapterformat}{%
\begingroup
\setlength{\unitlength}{1mm}%
\begin{picture}(20,40)(0,5)%
\setlength{\fboxsep}{0pt}%
%\put(0,0){\framebox(20,30){}}%
%\put(0,20){\makebox(20,20){\rule{20\unitlength}{20\unitlength}}}%
\put(20,15){\line(1,0){\dimexpr
\textwidth-20\unitlength\relax\@gobble}}%
\put(0,0){\makebox(20,20)[r]{%
\fontsize{28\unitlength}{1}\selectfont\thechapter
}}%
\put(20,15){\makebox(\dimexpr
\textwidth-20\unitlength\relax\@gobble,\ht\strutbox\@gobble)[l]{%
\ \normalsize\color{chapcolor}\chapapp~\thechapter\autodot
}}%
\end{picture} % <- the whitespace is intentional here
\endgroup
}%
\makeatother

\setcapindent{1em} % figure caption indent

\deffootnote[1em]{1em}{1em}{\textsuperscript{\thefootnotemark}}
%https://tex.stackexchange.com/questions/657471/scrbook-fixing-indentation-of-footnotes

